Unsupervised Enrichment of Persona-grounded Dialog with Background Stories

Humans often refer to personal narratives, life experiences, and events to make a conversation more engaging and rich. While persona-grounded dialog models are able to generate responses that follow a given persona, they often miss out on stating detailed experiences or events related to a persona, often leaving conversations shallow and dull. In this work, we equip dialog models with 'background stories' related to a persona by leveraging fictional narratives from existing story datasets (e.g. ROCStories). Since current dialog datasets do not contain such narratives as responses, we perform an unsupervised adaptation of a retrieved story for generating a dialog response using a gradient-based rewriting technique. Our proposed method encourages the generated response to be fluent (i.e., highly likely) with the dialog history, minimally different from the retrieved story to preserve event ordering and consistent with the original persona. We demonstrate that our method can generate responses that are more diverse, and are rated more engaging and human-like by human evaluators, compared to outputs from existing dialog models.

==> camera_ready_todo.tex <==
% Response: https://docs.google.com/document/d/1zk3oss8b5Viwhw4KYuKHcXgzcCu_WuUUmzoZ925xR-Q/edit
% Reviews: https://docs.google.com/document/d/1Udm7Q4pwlZEoBiuS3FixwOm6myU4BVwXJXDOBl-W8-0/edit
- 

- [done] add lamda exp details in experiment - Bodhi, done
- [done] add why did we use PABST instead PABST-peudo - Bodhi done
- [done] drop highlights from table 1 - Bodhi done
-  [done] resize table/equ to keep them in the margin - Bodhi done


- [done] IAA ratings
- [NA] clarify that PSEUDO means pabst pseudo or discchoice pseudo. same thing with Multitask. -- I think it is clarified in the baselines.
- [done] mention that ordering of outputs when performing human evals was randomized
- [todo] related work: had compressed a lot. can bring back some relevant references
- [done] can move human eval setup from appendix to main paper
- [done] briefly mention some more future directions ? perhaps with conclusion
    - some ideas about this: we always use the retrieved story, but can incorporate a decision to use or not. can use the retrieved text over multiple turns instead of single turn. 
- [done] results for pabst vs pabst-pseudo ? and a small discussion on how just changing decoding is good, but retraining models also helps
- [done] add one more example to main table ?
- [done] "We  also  experiment  with  different  values  of the  weight .. " - should we mention the number of samples tested ?. also can move the lambda experiment under a separate bold header than 'Human Evaluation' -- did subsectioning. 
- [done] add link to gihub repo. perhaps use a fresh blank repo for now-- as we still need to clean the code. -- added a placeholder in intro.tex
- [done] latest results in slack vs results in overleaf ?
- [done] "(1) Our early experiment shows that PABST and PABST-PSEUDO do .. (2)..since PABST does not require additional training whereas PABST-PSEUDO needs so to adapt to the story data..." - think the second point is enough. our main experiment/hypothesis is regarding decoding time availability of external corpora. so i would only keep (2) and delete (1) -- addressed.
- [todo] if its not too much, i think it will be worth adding a 'failure example', perhaps in appendix, showing an example where 


